On the Irrationality Exponents of Mahler Numbers

We explore Mahler numbers originating from functions $f(z)$ that satisfy the functional equation $f(z) = (A(z)f(z^d) + C(z))/B(z)$. A procedure to compute the irrationality exponents of such numbers is developed using continued fractions for formal Laurent series, and the form of all such irrationality exponents is investigated. This serves to extend Dmitry Badziahin's paper, On the Spectrum of Irrationality Exponents of Mahler Numbers, where he does the same under the condition that $C(z) = 0$. Furthermore, we cover the required background of continued fractions in detail for unfamiliar readers. This essay was submitted as a thesis in the Pure Mathematics Honours program at the University of Sydney.

==> chapters/extra_notes.tex <==
Currently using this chapter for notes on the gcd problem.\\
\\
\underline{Claim:} The degree of $\gcd(A(z)p_m(z^d)+C(z)q_m(z^d), B(z)q_m(z^d))$ is eventually cyclic.\\
\\
Without loss of generality, we may assume that $\deg(f) = 0$. Furthermore, assume that $r_a < r_c$, and hence $r_c = r_b$. Suppose that $B(z)$ is a product of irreducible polynomials, and that each of the factors has a root with absolute value greater than 1. Then the problem is solved.\\
\\
By the inclusion-exclusion principle and utilising the Euclidean algorithm,

\begin{align*}
&\gcd(A(z)p_m(z^d)+C(z)q_m(z^d), B(z)q_m(z^d))\\
&= \frac{\gcd(A(z)p_m(z^d)+C(z)q_m(z^d), B(z)) \gcd(A(z)p_m(z^d)+C(z)q_m(z^d), q_m(z^d))}{\gcd(A(z)p_m(z^d)+C(z)q_m(z^d), B(z), q_m(z^d))}\\
&= \frac{\gcd(A(z)p_m(z^d)+C(z)q_m(z^d), B(z)) \gcd(A(z), q_m(z^d))}{\gcd(A(z), B(z), q_m(z^d))}
\end{align*}

Now evaluating the first numerator term, let $z_0$ be a root of both arguments. Case 1: $A(z_0^{d^t}) \neq 0$ for all integer $t \geq 0$. Then,
\begin{align*}
\frac{p_m(z_0^d)}{q_m(z_0^d)} &= -\frac{C(z_0)}{A(z_0)}
\end{align*}
Now use the recursive definition of $p_m$ and $q_m$,
\begin{align*}
\frac{p_{m-1}(z^{d^2})}{q_{m-1}(z_0^{d^2})} &= -\frac{C(z_0)B(z_0^d)}{A(z_0)A(z_0^d)} - \frac{C(z_0^d)}{A(z_0^d)}
\end{align*}
repeating this until we reach $p_0$ and $q_0$,
\begin{align*}
\frac{p_0(z^{d^{m+1}})}{q_0(z^{d^{m+1}})} = -\sum_{k=0}^m \frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}
\end{align*}
As $|z_0| > 1$ and the degree of $\deg(p_0) = \deg(q_0)$, we have the LHS approaching a non-zero constant as $m \to \infty$. For the right hand side, we claim it diverges. This is because
\begin{align*}
\Big|\sum_{k=0}^m \frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| \geq \Big|\frac{C(z_0)}{A(z_0)} \prod_{i = 1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| - m\max_{1 \leq k \leq m} \Big(\Big|\frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big|\Big)
\end{align*}
note for the maximum term, we compare the degrees of the polynomials. The $k$-term has degree
\begin{align*}
&d^k(r_c-r_a) + \sum_{i=k+1}^m d^i (r_b-r_a)\\
&= d^k(r_c-r_a) + (r_b-r_a)\frac{d^{k+1}(d^{m-k}-1)}{d-1}\\
&= d^k(r_c-r_a) + \frac{(r_b-r_a)(d^{m+1}-d^{k+1})}{d-1}\\
&= \frac{(r_b-r_a)d^{m+1}}{d-1} + d^k(r_c-r_a-\frac{d(r_c-r_a)}{d-1})\\
&= \frac{(r_b-r_a)d^{m+1}}{d-1} - d^k(r_c-r_a)\frac{1}{d-1}
\end{align*}

So the degrees are increasing over $m$ and decreasing over $k$. As $m \to \infty$, the maximal degree term will dominate the smaller ones, hence eventually the largest term will be the $k = 0$ term, thus
\begin{align*}
\Big|\sum_{k=0}^m \frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| \geq \Big|\frac{C(z_0)}{A(z_0)} \prod_{i = 1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| - m\Big|\frac{C(z_0^d)}{A(z_0^d)} \prod_{i = 2}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big|
\end{align*}
again for large $m$, we will have $|z_0^m| > m$, hence
\begin{align*}
\Big|\sum_{k=0}^m \frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| \geq \Big|\frac{C(z_0)}{A(z_0)} \prod_{i = 1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| - \Big|\frac{C(z_0^d)z_0^m}{A(z_0^d)} \prod_{i = 2}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| 
\end{align*}

Again comparing the degrees of the terms, we will find the degree of the first term minus the second term is $d(r_b-r_a) > 0$, thus by asymptotic dominance again, eventually
\begin{align*}
\Big|\sum_{k=0}^m \frac{C(z_0^{d^k})}{A(z_0^{d^k})}\prod_{i = k+1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big| \geq \frac{1}{2}\Big|\frac{C(z_0)}{A(z_0)} \prod_{i = 1}^m \frac{B(z_0^{d^i})}{A(z_0^{d^i})}\Big|
\end{align*}

Taking $m \to \infty$, the infinite product will certainly diverge to $\infty$, hence there exists a $m_0 \in \N$ where we find a contradiction for $m \geq m_0$, thus $z_0$ cannot contribute to the GCD. Taking the maximum of the $m_0$ across all roots of $B(z)$ implies that eventually the GCD will be 1.\\
\\
Now for the other terms, 
\underline{Claim:} $\gcd(G(z), q_m(z^d))$ is eventually cyclic, where $G(z)$ is any polynomial.\\
\\
To prove this, we use the same approach as the paper. Just considering the non-cyclotomic terms, we know that eventually
\begin{align*}
\gcd(G(z), B(z^{d^t})) = 1.
\end{align*}
Now write 
\begin{align*}
q_m(z) = q'_{m}(z)\prod_{t=0}^{m-1} B_{t, m}(z) 
\end{align*}
where $q'_m(z) | q_0(z^{d^m})$, $B_{t, m}(z) | B(z^{d^t})$. Now note that there exists a $m_0$ where the $m \geq m_0$ parts don't contribute to the GCD, hence the GCD is only factors $B(z^{d^t})$ for $1 \leq t \leq m_0$. As there are a finite number of such factors, eventually the terms must repeat. (Now must show that the GCD only depends on the previous term) \\
\\



Test referencing the Mahler function \cite{badziahin} here.




